SurFhead: Affine Rig Blending for Geometrically Accurate 2D Gaussian Surfel Head Avatars

Recent advancements in head avatar rendering using Gaussian primitives have achieved significantly high-fidelity results. Although precise head geometry is crucial for applications like mesh reconstruction and relighting, current methods struggle to capture intricate geometric details and render unseen poses due to their reliance on similarity transformations, which cannot handle stretch and shear transforms essential for detailed deformations of geometry. To address this, we propose SurFhead, a novel method that reconstructs riggable head geometry from RGB videos using 2D Gaussian surfels, which offer well-defined geometric properties, such as precise depth from fixed ray intersections and normals derived from their surface orientation, making them advantageous over 3D counterparts. SurFhead ensures high-fidelity rendering of both normals and images, even in extreme poses, by leveraging classical mesh-based deformation transfer and affine transformation interpolation. SurFhead introduces precise geometric deformation and blends surfels through polar decomposition of transformations, including those affecting normals. Our key contribution lies in bridging classical graphics techniques, such as mesh-based deformation, with modern Gaussian primitives, achieving state-of-the-art geometry reconstruction and rendering quality. Unlike previous avatar rendering approaches, SurFhead enables efficient reconstruction driven by Gaussian primitives while preserving high-fidelity geometry.

==> NeRSemble_quanti_integrated.tex <==
\begin{wraptable}[11]{r}{5cm}
\scriptsize
    \setlength{\tabcolsep}{1.5pt}
    \vspace{2pt}
     \caption{\textbf{Quantitative comparison on NeRSemble.} 
     \colorbox{red!25}{Best} and \colorbox{yellow!25}{Second best}.}\label{wrap-tab:nersemble_quanti}
     \vspace{-5pt}
    \begin{tabular}{lcccc}
    \toprule
     & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$& NCS$\uparrow$ \\ 
    \midrule
    
    PointAvatar & &  & & \\
    FLARE &  & & \\
    SA &23.12 & 0.873 & 0.214 & \\
    GA &\cellcolor{yellow!25}23.42 &0.892&\cellcolor{red!25}0.092&\\
   
    % GA + 2DGS &   \cellcolor{yellow!25}23.4 & \cellcolor{yellow!25}0.893 & \cellcolor{yellow!25}0.105 \\
     \hline
    \textbf{Ours}              &   \cellcolor{red!25}23.53 & \cellcolor{red!25}0.904 & \cellcolor{yellow!25}0.099 &\\
     Ours + LPIPS              &   \cellcolor{red!25}23.53 & \cellcolor{red!25}0.904 & \cellcolor{yellow!25}0.099 &\\
    \bottomrule
    \vspace{-5pt}
    \end{tabular}
\end{wraptable} 


% \begin{table}[h]
% \centering
% \caption{Quantitative Comparison on FaceTalk synthetic dataset.}
% \label{tab:novel-view}
% \begin{tabular}{lcccc}
% \toprule

%  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & NCS $\uparrow$ \\
% \midrule
% IMAvatar & \cellcolor{yellow!25}29.5 & \cellcolor{green!25}0.913 & \cellcolor{red!25}0.152 \\
% PointAvatar  & \cellcolor{yellow!25}25.8 & \cellcolor{green!25}0.893 & \cellcolor{red!25}0.097 \\
% FLARE  & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% GaussianAvatars & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% Ours & \cellcolor{yellow!25}31.6 & \cellcolor{green!25}0.938 & \cellcolor{red!25}0.065 \\
% \bottomrule
% \end{tabular}
% \end{table}

==> NeRSemble_quanti_random.tex <==
\begin{wraptable}[8]{r}{5cm}
\scriptsize
    \setlength{\tabcolsep}{1.5pt}
    \vspace{-0pt}
     \caption{\textbf{Quantitative comparison on NeRSemble (random). } Red indicates the best and yellow the second.}\label{wrap-tab:nersemble_quanti}
    \begin{tabular}{lccc}
    \toprule
    & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\ 
    \midrule
    
    PointAvatar & &  &  \\
    FLARE &  & & \\
    SplattingAvatars &  &  & \\
    GaussianAvatars &\cellcolor{yellow!25}25.63&0.912&\cellcolor{red!25}0.080\\
   
    % GA + 2DGS &   \cellcolor{yellow!25}23.4 & \cellcolor{yellow!25}0.893 & \cellcolor{yellow!25}0.105 \\
     % \hline
    Ours              &    &  &  \\
    \bottomrule
    \end{tabular}
\end{wraptable} 


% \begin{table}[h]
% \centering
% \caption{Quantitative Comparison on FaceTalk synthetic dataset.}
% \label{tab:novel-view}
% \begin{tabular}{lcccc}
% \toprule

%  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & NCS $\uparrow$ \\
% \midrule
% IMAvatar & \cellcolor{yellow!25}29.5 & \cellcolor{green!25}0.913 & \cellcolor{red!25}0.152 \\
% PointAvatar  & \cellcolor{yellow!25}25.8 & \cellcolor{green!25}0.893 & \cellcolor{red!25}0.097 \\
% FLARE  & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% GaussianAvatars & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% Ours & \cellcolor{yellow!25}31.6 & \cellcolor{green!25}0.938 & \cellcolor{red!25}0.065 \\
% \bottomrule
% \end{tabular}
% \end{table}

==> ablation_deformation.tex <==
\begin{wraptable}[8]{r}{4.8cm}
\scriptsize
    \setlength{\tabcolsep}{0.9pt}
    \vspace{-10pt}
     \caption{\textbf{Ablations. \colorbox{red!25}{Best} and \colorbox{yellow!25}{Second best}.} +/- indicate incremental changes from the previous.}
     \label{wrap-tab:ablations}
    \begin{tabular}{lcccc}
    \toprule
     & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$& NCS$^p$ $\uparrow$ \\ 
    \midrule
    
    Vanilla  & 22.35   &  0.901  & 0.093 &  0.809 \\
    + Jacobian & 22.38   &  0.902  & 0.091 &  0.812 \\
    + JBS (= Ours) & \cellcolor{red!25} 23.09   & \cellcolor{red!25}0.931   & \cellcolor{red!25}0.082 & \cellcolor{yellow!25}0.845 \\
    \hline
    - ASGs & \cellcolor{yellow!25}
23.07   & 0.922   & 0.089 & \cellcolor{red!25}0.846 \\
    - eyeballs & 23.03   & \cellcolor{yellow!25}0.925   & \cellcolor{yellow!25}0.087 & 0.820 \\
    % - Eyeballs 
    \bottomrule
    \end{tabular}
\end{wraptable} 


% \begin{table}[h]
% \centering
% \caption{Quantitative Comparison on FaceTalk synthetic dataset.}
% \label{tab:novel-view}
% \begin{tabular}{lcccc}
% \toprule

%  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & NCS $\uparrow$ \\
% \midrule
% IMAvatar & \cellcolor{yellow!25}29.5 & \cellcolor{green!25}0.913 & \cellcolor{red!25}0.152 \\
% PointAvatar  & \cellcolor{yellow!25}25.8 & \cellcolor{green!25}0.893 & \cellcolor{red!25}0.097 \\
% FLARE  & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% GaussianAvatars & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% Ours & \cellcolor{yellow!25}31.6 & \cellcolor{green!25}0.938 & \cellcolor{red!25}0.065 \\
% \bottomrule
% \end{tabular}
% \end{table}

==> synthetic_quanti.tex <==
\begin{wraptable}[8]{r}{5cm}
\scriptsize
    \setlength{\tabcolsep}{2pt}
    \vspace{-15pt}
     \caption{\textbf{Comparison on FaceTalk~\cite{imavatar}.} \colorbox{red!25}{Best} and \colorbox{yellow!25}{Second best}}\label{wrap-tab:facetalk_quanti}
     \vspace{-8pt}
    \begin{tabular}{lcccc}
    \toprule
     & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & NCS $\uparrow$ \\ 
    \midrule
    
    IMAvatar  & 32.23   & 0.983  &  0.037 & 0.931\\
    PointAvatar & \cellcolor{yellow!25}34.93 & \cellcolor{yellow!25}0.984 & 0.065 & 0.756 \\
    FLARE & 31.64 & 0.968& \cellcolor{yellow!25}0.027 & \cellcolor{yellow!25}0.943 \\
    \hline
    % 2DGA &   \cellcolor{yellow!25}39.7 & \cellcolor{yellow!25}0.991 & \cellcolor{yellow!25}0.021 & \cellcolor{yellow!25} 0.980  \\
    \textbf{Ours}              &   \cellcolor{red!25}40.15 & \cellcolor{red!25}0.992 & \cellcolor{red!25}0.020 & \cellcolor{red!25}0.983 \\
    \bottomrule
    \end{tabular}
\end{wraptable} 


% \begin{table}[h]
% \centering
% \caption{Quantitative Comparison on FaceTalk synthetic dataset.}
% \label{tab:novel-view}
% \begin{tabular}{lcccc}
% \toprule

%  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & NCS $\uparrow$ \\
% \midrule
% IMAvatar & \cellcolor{yellow!25}29.5 & \cellcolor{green!25}0.913 & \cellcolor{red!25}0.152 \\
% PointAvatar  & \cellcolor{yellow!25}25.8 & \cellcolor{green!25}0.893 & \cellcolor{red!25}0.097 \\
% FLARE  & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% GaussianAvatars & \cellcolor{yellow!25}26.7 & \cellcolor{green!25}0.899 & \cellcolor{red!25}0.122 \\
% Ours & \cellcolor{yellow!25}31.6 & \cellcolor{green!25}0.938 & \cellcolor{red!25}0.065 \\
% \bottomrule
% \end{tabular}
% \end{table}
